MAIR: A Massive Benchmark for Evaluating Instructed Retrieval

Recent information retrieval (IR) models are pre-trained and instruction-tuned on massive datasets and tasks, enabling them to perform well on a wide range of tasks and potentially generalize to unseen tasks with instructions. However, existing IR benchmarks focus on a limited scope of tasks, making them insufficient for evaluating the latest IR models. In this paper, we propose MAIR (Massive Instructed Retrieval Benchmark), a heterogeneous IR benchmark that includes 126 distinct IR tasks across 6 domains, collected from existing datasets. We benchmark state-of-the-art instruction-tuned text embedding models and re-ranking models. Our experiments reveal that instruction-tuned models generally achieve superior performance compared to non-instruction-tuned models on MAIR. Additionally, our results suggest that current instruction-tuned text embedding models and re-ranking models still lack effectiveness in specific long-tail tasks. MAIR is publicly available at https://github.com/sunnweiwei/Mair.

==> SIGIR.tex <==
\subsection{SIGIR}\label{SIGIR}
\subsubsection{ACORDAR}
The paper studies the task of ad hoc content-based dataset retrieval. Keyword queries are used to retrieve datasets, where the target documents are the metadata and data content of the datasets. 

\begin{itemize}
    \item The queries come in two forms: synthetic and TREC queries. 
    Synthetic queries are created by human annotators by summarizing the content of a dataset they browsed, aiming to match the dataset's content. 
    TREC queries are general topic queries from the TREC test collections.
    \item The documents are datasets containing metadata (e.g. title, description, author) and data content (RDF triples). 
    These datasets are from 543 open data portals across multiple domains, in the RDF data format. 
    The datasets vary greatly in data size and schema size.
    \item Relevance is judged based on whether the information contained in a dataset would be used when writing a report or developing an application on the topic of the query. 
    The relevance is divided into 3 levels:
    \begin{itemize}
        \item Irrelevant(0): the dataset is completely unrelated to the query topic, and none of its information would be used.
        \item Partially relevant(1): the dataset has some content related to the query topic, and some of its information may be used, but not all.
        \item Highly relevant(2): the dataset is highly related to the query topic, and much of its contained information would be heavily used. It can largely satisfy the information needs of the query.
    \end{itemize}
    \item We annotate instructions like this "Given a question, identify and retrieve datasets where the keywords in the query may be found in either the metadata or the actual data of the dataset."
\end{itemize}

\subsubsection{ChroniclingAmericaQA}
This paper studies the open-domain question-answering task, using natural language questions as queries to retrieve relevant answers from the Chronicling America collection of historical American newspaper pages.

\begin{itemize}
    \item The queries used are natural language questions, such as "How many subscribers did Jackson lose on Saturday?". 
    These questions are automatically generated based on the content of the newspaper articles.
    \item The document collection used for retrieval is the Chronicling America collection of historical American newspapers. 
    It is a large digital archive containing over 21 million pages of newspapers published between 1756 and 1963, covering information ranging from major historical events to everyday life details. 
    The documents are available in both scanned image and OCR text formats.
    \item The ChroniclingAmericaQA dataset uses a binary relevance classification:
    \begin{itemize}
        \item Relevant(1): The answer comes from the given historical newspaper document collection and is semantically relevant to the question, providing an answer to the query.
        \item Not Relevant(0): The answer does not come from the given document collection, or even if it does, it is semantically unrelated to the question and cannot answer the query.
    \end{itemize}
    \item We annotate instructions like this "Given a question, retrieve newspaper pages that contain the answer to the question from the American historical newspaper dataset Chronicling America."
\end{itemize}

\subsubsection{CPCD}
This paper studies a new retrieval task called Conversational Item Set Curation. In this task, a user engages in a conversation with a system to curate a small set of items (e.g. a music playlist) from a larger collection. The system needs to retrieve relevant items (e.g. songs) based on the conversation history and recommend them to the user.

\begin{itemize}
    \item The query is formed from the conversation history, comprising all previous user utterances. 
    For example, the user may first state a theme ("Create a rock playlist for a long drive"), and then provide additional details and preferences in subsequent turns ("Do you have anything from old Stevie Wonder?").
    \item The documents are the items in the collection to be retrieved, which in this work are songs. 
    Each song is represented as a text document in the format "<title> by <artist> from <album>". The song data comes from expert-curated playlist descriptions.
    \item Relevance is judged based on the preferences expressed by the user during the conversation. 
    A song is considered relevant if it matches the theme, genre, artist, etc. mentioned by the user. 
    The relevance is divided into 4 levels:
    \begin{itemize}
        \item Highly relevant(3): Matches all preferences expressed by the user
        \item Relevant(2): Matches most of the preferences expressed
        \item Partially relevant(1): Matches some of the preferences expressed
        \item Not relevant(0): Does not match any of the expressed preferences
    \end{itemize}
    \item We annotate instructions like this "The query is a dialogue history in which the user seeks music recommendations. In each turn, the system recommends some music, and the user provides feedback indicating whether they like or dislike the recommendations. Based on the user's preferences and requests, retrieve music that the user is likely to enjoy as the recommendation response."
\end{itemize}

\subsubsection{Monant}
This paper studies the task of detecting medical misinformation. Specifically, given a fact-checked medical claim, it aims to retrieve news articles or blog posts that contain that claim.

\begin{itemize}
    \item The queries used are fact-checked medical claims, e.g. "Omega-3 fatty acids decrease triglycerides".
    \item The documents being retrieved are medical news articles and blog posts. These articles come from multiple reliable and unreliable website sources and include text content, images, videos, etc. The data is collected from the web using web crawlers.
    \item The basis for relevance levels is whether the article contains the given claim, and what stance the article takes towards that claim (supporting, contradicting, or neutral). The relevance levels are:
    \begin{itemize}
        \item Present(1): The article contains a sentence or paragraph that is literally or semantically similar to the claim
        \item Not present(2): The article does not contain the claim
        \item Supporting(3) The article supports the claim
        \item Contradicting(4) The article contradicts the claim
        \item Neutral(5) The article has a neutral stance toward the claim
    \end{itemize}
    \item We annotate instructions like this "Given a medical claim, retrieve articles that either support or contradict the claim."
\end{itemize}

\subsubsection{NTCIR}
The paper introduces a new test collection for ad-hoc dataset retrieval. The task is to retrieve relevant datasets from open government data portals (Data.gov and e-Stat) given a query derived from real information needs. 


\begin{itemize}
    \item The queries are keyword queries transformed from real information needs, aiming to capture users' actual search intents.
    \item The documents being retrieved are datasets from the government's open data portals, where each dataset contains metadata and one or more data files, mainly from Data.gov (US) and e-Stat (Japan) covering various domains.
    \item Relevance judgments are based on how useful a dataset is for satisfying the information need behind the query, with 3 grades:
    \begin{itemize}
        \item Irrelevant(0): The dataset is completely irrelevant to the query.
        \item Partially relevant(1): The dataset contains some relevant content but cannot fully satisfy the need.
        \item Highly relevant(2) The dataset can well satisfy the information need of the query.
    \end{itemize}
    \item We annotate instructions like this "Given a search query, retrieve relevant datasets from Data.gov and e-Stat that contain the requested information."
\end{itemize}

\subsubsection{PointRec}
This paper studies a point-of-interest (POI) recommendation task driven by natural language descriptions. User queries are natural language descriptions of their travel needs and preferences, which are used to retrieve from a document collection of 695,000 POI entries.

\begin{itemize}
    \item The queries are in the form of natural language descriptions, specifying the user's travel destination, preferred categories (e.g. restaurants, nightlife), travel group, specific requirements or constraints on the POIs, etc. For example, "I want to find a not-too-noisy restaurant with good service near London to take my 80-year-old dad for a meal."
    \item The document collection contains 695,000 POI entries collected from Yelp's online directory, spanning over 2,000 cities across 23 countries. Each POI entry includes basic information like name, address, categories, rating, and review count, and is linked to the GeoNames geographical knowledge base for location data. Relevant text snippets are also extracted from web search results as descriptions. So this is a cross-domain document collection containing both structured data and unstructured text.
    \item The relevance judgments are primarily based on whether the POI satisfies the destination, category, travel group, and specific requirements or constraints described in the query. The relevance levels are:
    \begin{itemize}
        \item Highly relevant(3): The POI perfectly matches the location, category, and all constraints specified in the query
        \item Relevant(2): The location and category match and the requester would likely be interested
        \item Somewhat relevant(1): The location matches, and the requester could possibly be interested  
        \item Not relevant(0): The POI does not satisfy any of the above conditions
    \end{itemize}
    \item We annotate instructions like this "Given a user's request, recommend a point of interest (POI) that best matches the user's intent. Use the following metadata for reference:{'Group': xx, 'Main Category': xx, 'Sub Categories': [xx, ...], ...}"
\end{itemize}
\subsubsection{ProCIS}
The paper studies the task of proactive retrieval, where the system proactively retrieves and recommends documents relevant to an ongoing multi-party conversation, without the user explicitly providing a query. The query is the entire conversation history, and the documents are from Wikipedia articles.

The paper studies two different tasks:

Turn-level Proactive Retrieval: In this task, the system needs to decide whether to retrieve documents at each turn of the conversation. If it decides to retrieve, it needs to return a ranked list of documents as contextual suggestions for that turn.

Dialog-level Reactive Retrieval: In this task, the system needs to retrieve relevant documents based on the entire conversation history after the conversation is finished, as contextual suggestions for the whole dialogue.

\begin{itemize}
    \item The query is the full context history of an ongoing multi-party human-machine conversation. The system needs to understand the conversation context and proactively retrieve documents relevant to the conversation at opportune moments as suggestions.
    \item The documents are articles from Wikipedia, covering a wide range of topics such as politics, religion, sports, finance, science, etc. These documents can provide useful background information, context, or supplementary knowledge for the ongoing conversation. The data source is Reddit conversation threads, which are cleaned and augmented by linking to Wikipedia articles.
    \item The basis for relevance levels is the degree to which the document is associated with the conversation, i.e., how much useful background information and context the document provides for the conversation.
    There are 3 relevance levels:
    \begin{itemize}
        \item Provides Useful Context (2): The document is directly related to the conversation, providing substantial useful background information or supplementary knowledge that enhances the understanding of the conversation.
        \item Partially Relevant (1): The document is somewhat related to the conversation. It provides some context or additional information but is not directly tied to the main topic of the conversation.
        \item Irrelevant (0): The document is completely unrelated to the conversation and does not provide any useful context or additional information.
    \end{itemize}
    \item We annotate instructions like this "Given a multi-party human conversation (such as a Reddit post and its comments), retrieve relevant documents from Wikipedia to provide contextual information. The criteria for relevance are as follows: ..."
\end{itemize}

\subsubsection{QuanTemp}
This paper studies the retrieval task for numerical claims for fact-checking. It uses the original claims and questions generated from claim decomposition as queries to retrieve relevant evidence documents from the web.

\begin{itemize}
    \item The queries include the original numerical claims as well as a series of questions decomposed from the claims using methods like ClaimDecomp and Program-FC. For example, for the claim "The ICE spends 4 times the amount to detain a person for a year than on a student in public school", the decomposed questions could include "How much does ICE spend to detain a person for a year?", "How much is spent on a student in public school?" etc.
    \item The documents are relevant to web page snippets retrieved from the internet, covering domains like Wikipedia, government websites, statistics websites, etc. These snippets do not include any content from fact-checking websites to prevent the model from learning shortcuts. A total of 423,320 such evidence snippets are collected.
    \item The relevance levels are classified based on the usefulness of the evidence snippets in verifying the original claim.
    The relevance levels are as follows:
    \begin{itemize}
        \item Highly relevant(3): Evidence snippet directly supports or refutes the claim
        \item Partially relevant(2): Evidence snippet contains information helpful in verifying parts of the claim
        \item Not relevant(1): The evidence snippet is not related to the claim
        \item Contradictory(0): Evidence snippet contradicts the claim
    \end{itemize}
    \item We annotate instructions like this "Given a numerical claim, retrieve documents that can verify the claim."
\end{itemize}

% \subsubsection{RecMeApp}
% This paper studies the task of mobile app recommendation. It does not use queries to retrieve documents. Instead, it constructs a large-scale dataset called MobileRec containing user interactions with mobile apps, which is used to train and evaluate recommendation models.

% \begin{itemize}
%     \item No query
%     \item The document refers to the MobileRec dataset, which contains 19.3 million user reviews and ratings for mobile apps from the Google Play Store, covering 10,173 distinct apps across 48 categories. Each record includes rich information such as user ID, app details, review text, rating score, and timestamp. It is a large-scale sequential user-app interaction dataset.
%     \item The relevance levels are as follows:
%     \begin{itemize}
%         \item Highly relevant(3): The recommendation system performs excellently on the evaluation metrics for this dataset.
%         \item Moderately relevant(2): The recommendation system has average performance on the evaluation metrics for this dataset. 
%         \item Slightly relevant(1): The recommendation system performs poorly on the evaluation metrics for this dataset.
%         \item Not relevant(0): The recommendation system completely fails to work well on this dataset.
%     \end{itemize}
% \end{itemize}

\subsubsection{WebTableSearch}
This paper studies the task of web table retrieval. It uses keyword queries to retrieve a set of relevant web tables.


\begin{itemize}
    \item The query is a set of keywords describing the user's information need, e.g. "Fast cars".
    \item The documents are HTML tables extracted from the Common Crawl web corpus. These tables are from 61,086 different domain names, covering a broad range of topics. In addition to the table itself, each table has associated context fields such as page title, text before/after the table, and entities linked to DBpedia.
    \item The relevance levels are judged based on how relevant the query is to the table and its context fields (e.g. page title, surrounding text).
    There are 3 relevance levels:
    \begin{itemize}
        \item Not relevant(0): This field is not relevant to the query.
        \item Relevant (1): This field provides relevant information about the query.
        \item Highly relevant (2): This field provides ideal information about the query.
    \end{itemize}
    \item We annotate instructions like this "Given a question, retrieve relevant table to answer the question."
\end{itemize}














==> table/all_task.tex <==
\begin{table*}[h]
\centering\small
\setlength\tabcolsep{2pt}
\caption{List of tasks in \textsc{Mair}.}
\label{table:list-tasks-1}
\begin{tabular}{l cccccc}
\toprule
\textbf{Task} & Reference & Query & Doc & Task Type & Domain\\
\midrule

Competition-Math &  \citet{Hendrycks2021MeasuringMP} & Math question & Answer & Question Answering & Academic\\
ProofWiki\_Proof & \citet{Welleck2021NaturalProofsMT} & Math Statement & Proof & Proof Retrieval & Academic\\
Stacks\_Proof & \citet{Welleck2021NaturalProofsMT} & Math Statement & Proof & Proof Retrieval & Academic\\
Stein\_Proof & \citet{Welleck2021NaturalProofsMT} & Math Statement & Proof & Proof Retrieva & Academic\\
Trench\_Proof & \citet{Welleck2021NaturalProofsMT} & Math Statement & Proof & Proof Retrieval & Academic\\
ProofWiki\_Reference & \citet{Welleck2021NaturalProofsMT} & Math Statement & Reference & Reference Retrieval & Academic\\
Stacks\_Reference & \citet{Welleck2021NaturalProofsMT} & Math Statement & Reference & Reference Retrieval & Academic\\
Stein\_Reference & \citet{Welleck2021NaturalProofsMT} & Math Statement & Reference & Reference Retrieval & Academic\\
Trench\_Reference & \citet{Welleck2021NaturalProofsMT} & Math Statement & Reference & Reference Retrieval & Academic\\
TAD & \citet{Chen2022TargetawareAR} & Paper Abstract & Citation & Reference Retrieval & Academic\\
TAS2 & \citet{Chen2022TargetawareAR} & Paper Abstract & Citation & Reference Retrieval & Academic\\
StackMathQA & \citet{Chen2022TargetawareAR} & Math Question & Answer & Question Answering & Academic\\

\midrule
APPS & \citet{Hendrycks2021MeasuringCC} & Code Problem & Solution & Code Retrieval & Code\\
CodeEditSearch & \citet{Muennighoff2023OctoPackIT} & Commit & Code Diff & Code Retrieval & Code\\
CodeSearchNet & \citet{Husain2019CodeSearchNetCE} & Function Header & Function & Code Retrieval & Code\\
HumanEval-X & \citet{Zheng2023CodeGeeXAP} & Code Problem & Solution & Code Retrieval & Code\\
LeetCode & \href{https://huggingface.co/datasets/greengerong/leetcode}{LeetCode} & Code Problem & Solution & Code Retrieval & Code\\
MBPP & \citet{Austin2021ProgramSW} & Code Problem & Solution & Code Retrieval & Code\\
Conala & \citet{Zhou2022DocPromptingGC} & NL Command & Command Doc & Code Retrieval & Code\\
TLDR & \citet{Zhou2022DocPromptingGC} & CNL Command & Command Doc & Code Retrieval & Code\\
RepoBench & \citet{Liu2023RepoBenchBR} & Code Context & Next Function &  GitHub Agent & Code\\
SWE-Bench & \citet{Jimenez2023SWEbenchCL} & GitHubIssue & Related File & GitHub Agent & Code\\

\midrule

Apple & \href{https://huggingface.co/datasets/lighthouzai/finqabench}{FinQabench} & Question & Paragraph & Question Answering & Finance\\
ConvFinQA & \citet{Chen2022ConvFinQAET} & Dialog & Table \& Paragraph & Dialog Retrieval & Finance\\
FinQA & \citet{Chen2021FinQAAD} & Question & Paragraph & Question Answering & Finance\\
FinanceBench & \citet{Islam2023FinanceBenchAN} & Question & Pages & Question Answering & Finance\\
HC3Finance & \href{https://huggingface.co/datasets/Atharva07/hc3_finance}{HC3Finance} & Question & Answer & Question Answering & Finance\\
TAT-DQA & \citet{Zhu2022TowardsCD} & Question & Table \& Paragraph & Question Answering & Finance\\
Trade-the-event & \href{https://huggingface.co/datasets/nickmuchi/trade-the-event-finance}{Trade-the-event} & Title & Article & Summary Retrieval & Finance\\

\midrule
ELI5 & \citet{Fan2019ELI5LF} & Question & Passages & Question Answering & Web\\
Fever & \citet{Thorne2018FEVERAL} & Claim & Passages & Fact Checking & Web\\
AY2 & \citet{Hoffart2011RobustDO} & Entity Mention & Entity Page & Entity Linking & Web\\
WnCw & \citet{Guo2018RobustNE} & Entity Mention & Entity Page & Entity Linking & Web\\
WnWi & \citet{Guo2018RobustNE} & Entity Mention & Entity Page & Entity Linking & Web\\
TREx & \citet{ElSahar2018TRExAL} & Entity \& Relation & Entity Page & Slot Filling & Web\\
zsRE & \citet{Levy2017ZeroShotRE} & Entity \& Relation & Entity Page & Slot Filling & Web\\
WoW & \citet{Dinan2018WizardOW} & Dialog & Passage & Dialog Retrieval & Web\\


\midrule
AILA2019-Case & \citet{Bhattacharya2019OverviewOT} & Situation & Prior Case & Case Retrieval & Legal\\
AILA2019-Statutes & \citet{Bhattacharya2019OverviewOT} & Situation & Statute & Statue Retrieval & Legal\\
BSARD & \citet{Louis2021ASA} & Question & Statute & Statue Retrieval & Legal\\
BillSum & \citet{Kornilova2019BillSumAC} & Summary & Article & Summary Retrieval & Legal\\
CUAD & \citet{Hendrycks2021CUADAE} & Instruction & Highlight & Contract Review & Legal\\
GerDaLIR & \citet{Wrzalik2021GerDaLIRAG} & Legal Case & Prior Cases & Case Retrieval & Legal\\
LeCaRDv2 & \citet{Li2023LeCaRDv2AL} & Legal Case & Prior Cases & Case Retrieval & Legal\\
LegalQuAD & \citet{Hoppe2021TowardsIL} & Question & Statute & Statute Retrieval & Legal\\
REGIR-EU2UK & \citet{Chalkidis2021RegulatoryCT} & EU Directive & UK Legislation & Statute Retrieval & Legal\\
REGIR-UK2EU & \citet{Chalkidis2021RegulatoryCT} & UK Legislation & EU Directive & Statute Retrieval & Legal\\


\midrule
ArguAna & \citet{Wachsmuth2018RetrievalOT} & Claim & Document & Argument Retrieval & Web\\
CQADupStack & \citet{Hoogeveen2015CQADupStackAB} & Question & Duplicate Question & Query Retrieval & Web\\
FiQA & \citet{Maia2018WWW18OC} & Question & Answer & Question Answering & Finance\\
NFCorpus & \citet{Boteva2016AFL} & Question & Medical Document & Medical QA & Medical\\
Quora & \href{https://huggingface.co/datasets/mteb/quora}{Quora} & Question & Duplicate Question & Query Retrieval & Web\\
SciDocs & \citet{Cohan2020SPECTERDR} & Paper Title & Citation & Reference Retrieval & Academic\\
SciFact & \citet{Wadden2020FactOF} & Claim & Document & Fact Checking & Academic\\
TopiOCQA & \citet{Adlakha2021TopiOCQAOC} & Dialog & Passage & Dialog Retrieval & Web\\
Touche & \citet{Bondarenko2020OverviewOT} & Question & Passages & Argument Retrieval & Web\\
Trec-Covid & \citet{Roberts2020TRECCOVIDRA} & Medical Question & Answer & Medical QA & Medical\\
\bottomrule
\end{tabular}
\end{table*}



\begin{table*}[h]
\centering\small
\setlength\tabcolsep{2pt}
\caption{List of tasks in \textsc{Mair}.}
\label{table:list-tasks-2}
\begin{tabular}{l cccccc}
\toprule
\textbf{Task} & Reference & Query & Doc & Task Type & Domain \\
\midrule
ACORDAR & \citet{Lin2022ACORDARAT} & Request & Dataset & Dataset Retrieval & Web\\
CPCD & \citet{Chaganty2023BeyondSI} & Dialog & Music & Recommendation & Web\\
ChroniclingAmericaQA & \citet{Piryani2024ChroniclingAmericaQAAL} & Question & News & News Retrieval & Web\\
Monant & \citet{Srba2022MonantMM} & Medical Claim & Document & Question Answering & Medical\\
NTCIR & \citet{Kato2021ATC} & Key Words & Dataset & Dataset Retrieval & Web\\
PointRec & \citet{Afzali2021POINTRECAT} & Question & POI & Recommendation & Web\\
ProCIS-Dialog & \citet{Samarinas2024ProCISAB} & Dialoge & Passage & Dialog Retrieval & Web\\
ProCIS-Turn & \citet{Samarinas2024ProCISAB} & Utterance & Passage & Dialog Retrieval & Web\\
QuanTemp & \citet{Venktesh2024QuanTempAR} & Numerical Claim & Document & Fact Checking & Web\\
WebTableSearch & \citet{Chen2021WTRAT} & Question & Table & Table Retrieval & Web\\

\midrule
CAsT & \href{ttps://www.treccast.ai}{TREC CAsT} & Dialog & Passage & Dialog Retrieval & Web\\
CliniDS\_2014 & \href{https://www.trec-cds.org/2014.html}{TREC CDS 2014} & Medical Case & Articles & Medical IR & Medical\\
CliniDS\_2015 & \href{https://www.trec-cds.org/2015.html}{TREC CDS 2015} & Medical Case & Articles & Medical IR & Medical\\
CliniDS\_2016 & \href{https://www.trec-cds.org/2016.html}{TREC CDS 2016} &  Health Record & Articles & Medical IR & Medical\\
ClinicalTrials\_2021 & \href{https://www.trec-cds.org/2021.html}{TREC CDS 2021} &  Health Record & Clinical Trials & Medical IR & Medical\\
ClinicalTrials\_2022 & \href{https://www.trec-cds.org/2022.html}{TREC CDS 2022} &  Health Record & Clinical Trials & Medical IR & Medical\\
ClinicalTrials\_2023 & \href{https://www.trec-cds.org/2023.html}{TREC CDS 2023} &  Patient Description & Clinical Trials & Medical IR & Medical\\
DD\_2015 & \href{https://trec.nist.gov/data/domain2015.html}{Domain2015} & Topic & Document & Web Search & Web\\
DD\_2016 & \href{https://trec.nist.gov/data/domain2016.html}{Domain2016} & Topic & Document & Web Search & Web\\
DD\_2017 & \href{https://trec.nist.gov/data/domain2016.html}{Domain2017} & Topic & Document & Web Search & Web\\
FairRanking\_2020 & \href{https://fair-trec.github.io/}{Fair-TREC} & Key Words & Academic Articles & Web Search & Academic\\
FairRanking\_2021 & \href{https://fair-trec.github.io/}{Fair-TREC} & WikiProject & Wikipedia Page & Web Search & Web\\
FairRanking\_2022 & \href{https://fair-trec.github.io/}{Fair-TREC} & WikiProject & Wikipedia Page & Web Search & Web\\
Genomics-AdHoc\_2004 & \href{https://trec.nist.gov/data/genomics.html}{Genomics} &  Question & Document & Medical IR & Medical\\
Genomics-AdHoc\_2005 & \href{https://trec.nist.gov/data/genomics.html}{Genomics} &  Question & Document & Medical IR & Medical\\
Genomics-AdHoc\_2006 & \href{https://trec.nist.gov/data/genomics.html}{Genomics} &  Question & Document & Medical IR & Medical\\
Genomics-AdHoc\_2007 & \href{https://trec.nist.gov/data/genomics.html}{Genomics} &  Question & Entity \& Passages & Medical IR & Medical\\
TREC-Legal\_2011 & \href{https://trec-legal.umiacs.umd.edu/}{TREC Legal} & Request & Communications & Case Retrieval & Legal\\
NeuCLIR-Tech & \href{https://neuclir.github.io/}{NeuCLIR} & Question & Document & Web Search & Web\\
NeuCLIR\_2022 & \href{https://neuclir.github.io/}{NeuCLIR} & Question & Document & Web Search & Web\\
NeuCLIR\_2023 & \href{https://neuclir.github.io/}{NeuCLIR} & Question & Document & Web Search & Web\\
ProductSearch\_2023 & \href{https://trec-product-search.github.io/index.html}{TREC Product Search} & Key Words & Product & Product Search & Web\\
ToT\_2023 & \href{https://trec-tot.github.io/}{TREC ToT} & Description & Wikipedia Page & Tip-of-the-Tongue & Web\\
ToT\_2024 & \href{https://trec-tot.github.io/}{TREC ToT} & Description & Wikipedia Page & Tip-of-the-Tongue & Web\\
Microblog & \href{https://github.com/ngc7023/TREC-Microblog-Datasets}{TREC Microblog} & Topic & Tweet & Tweet Retrieval & Web \\
PM & \href{https://trec.nist.gov/data/precmed.html}{Precision Medicine} & Patient Data & Clinical Trials & Medical IR & Medical\\
PM-Article & \href{https://trec.nist.gov/data/precmed.html}{Precision Medicine} & Patient Data & Articles & Medical IR & Medical\\
\midrule
CARE & \citet{Yang2024CAREAB} & Reaction & Proteins Documents & Medical IR & Medical \\
MISeD & \citet{Golany2024EfficientDG} & Dialog & Meeting Transcript & Meeting Retrieval & Web \\
SParC & \citet{Yu2019SParCCS} & Question & Table & Table Retrieval & Web\\
SParC-SQL & \citet{Yu2019SParCCS} & SQL Statement & Table & Table Retrieval & Web\\
Spider & \citet{Yu2018SpiderAL} & Question & Table & Table Retrieval & Web \\
Spider-SQL & \citet{Yu2018SpiderAL} & SQL Statement & Table & Table Retrieval & Web  \\
LitSearch & \citet{Ajith2024LitSearchAR} & Question & Articles & Literature Search & Academic \\
FoodAPI & \citet{shi2024chain}  & Question & Food API & Tool Retrieval & Code \\
TensorAPI  & \citet{patil2023gorilla}  & Question & Tensor API & Tool Retrieval & Code \\
HF-API & \citet{patil2023gorilla}  & Question & Huggingface API & Tool Retrieval & Code \\
PyTorchAPI & \citet{patil2023gorilla}  & Question & PyTorch API & Tool Retrieval & Code  \\
SpotifyAPI  & \citet{shi2024chain}  & Question & Spotify API & Tool Retrieval & Code  \\
TMDB  & \citet{shi2024chain}  & Question & TMDB API & Tool Retrieval & Code  \\
WeatherAPI  & \citet{shi2024chain}  & Question & Weather API & Tool Retrieval & Code \\
% APISearch & \citet{Shen2023HuggingGPTSA} & Question & Huggingface API & Tool Retrieval & Code\\
% Web APISearch & \citet{shi2024chain} & Question & Web API & Tool Retrieval & Code\\
ToolBench & \citet{Qin2023ToolLLMFL} & Question & Tool & Tool Retrieval & Code\\
ExcluIR & \citet{Zhang2024ExcluIREN} & Question & Passage & Negative Retrieval & Web\\
FollowIR\_Core17 & \citet{weller2024followir} & Question & Document & Negative Retrieval & Web\\
FollowIR\_News21 & \citet{weller2024followir} & Question & News & Negative Retrieval & Web\\
FollowIR\_Robust04 & \citet{weller2024followir} & Question & News & Negative Retrieval & Web\\
InstructIR & \citet{oh2024instructir} & Question & Passage & Web Search & Web\\
NevIR & \citet{Weller2023NevIRNI} & Question & Passage & Negative Retrieval & Web\\
IFEval & \citet{Zhou2023InstructionFollowingEF} & Question & Answer & Question Answering & Web\\
\bottomrule
\end{tabular}
\end{table*}



==> table/hard_set.tex <==
\begin{table*}[h]
\centering\tiny
\setlength\tabcolsep{2pt}
\caption{Results.}
\label{table:all-results}
\begin{tabular}{l cc cc cc cc cc cc cc cc cc cc}

\toprule
\textbf{Model} & \multicolumn{2}{c}{\textbf{Stacks\_Ref}} & \multicolumn{2}{c}{\textbf{RepoBench}} & \multicolumn{2}{c}{\textbf{TLDR}} & \multicolumn{2}{c}{\textbf{SWE-Bench}} & \multicolumn{2}{c}{\textbf{AILA-Case}} & \multicolumn{2}{c}{\textbf{AILA-Statutes}} & \multicolumn{2}{c}{\textbf{CUAD}} & \multicolumn{2}{c}{\textbf{LeCaRDv2}} & \multicolumn{2}{c}{\textbf{REGIR-UK2EU}} & \multicolumn{2}{c}{\textbf{Touche}} \\
\midrule
Instruction? & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} \\
\midrule
BM25 & 24.18 & - & 7.06 & - & 10.76 & - & 56.69 & - & 13.20 & - & 11.03 & - & 23.03 & - & 58.98 & - & 64.97 & - & 59.03 & - \\
\midrule

\code{contriever-msmarco} & 20.31 & - & 7.44 & - & 15.59 & - & 32.58 & - & 10.27 & - & 9.10 & - & 21.85 & - & 47.67 & - & 44.34 & - & 42.55 & - \\
\code{gtr-t5-base} & 16.68 & - & 14.09 & - & 15.17 & - & 40.47 & - & 4.69 & - & 9.84 & - & 20.91 & - & 41.16 & - & 44.27 & - & 48.05 & - \\
\code{gtr-t5-large} & 17.80 & - & 14.73 & - & 19.63 & - & 41.49 & - & 4.83 & - & 12.96 & - & 24.57 & - & 48.40 & - & 40.69 & - & 53.06 & - \\
\midrule

\code{all-MiniLM-L6-v2} & 20.32 & 21.14 & 11.56 & 4.87 & 15.60 & 7.39 & 35.18 & 32.09 & 6.54 & 5.76 & 11.71 & 7.24 & 23.03 & 8.55 & 43.01 & 36.93 & 31.53 & 31.01 & 35.06 & 29.40 \\
\code{e5-small-v2} & 21.66 & 19.48 & 11.79 & 9.72 & 12.92 & 5.54 & 38.64 & 35.39 & 7.60 & 6.43 & 10.41 & 7.52 & 22.92 & 15.05 & 46.16 & 44.05 & 30.43 & 32.31 & 39.49 & 41.75 \\
\code{e5-base-v2} & 23.44 & 21.94 & 8.72 & 9.53 & 15.63 & 10.17 & 46.07 & 46.91 & 8.27 & 5.65 & 10.59 & 8.38 & 22.94 & 19.51 & 42.18 & 41.51 & 39.79 & 41.67 & 41.10 & 40.26 \\
\code{e5-large-v2} & 22.87 & 21.63 & 10.30 & 7.89 & 17.58 & 11.34 & 42.71 & 37.69 & 11.85 & 9.15 & 8.41 & 7.75 & 27.94 & 20.03 & 51.15 & 47.97 & 36.80 & 36.26 & 34.80 & 33.59 \\
\code{gte-base-en-v1.5} & 23.11 & 20.16 & 12.53 & 5.17 & 13.53 & 3.28 & 49.60 & 44.96 & 11.53 & 9.77 & 13.74 & 12.13 & 25.97 & 21.17 & 50.28 & 50.32 & 43.11 & 44.95 & 45.78 & 33.69 \\
\code{gte-large-en-v1.5} & 22.72 & 22.66 & 11.43 & 1.95 & 13.75 & 2.05 & 47.93 & 37.28 & 9.03 & 7.54 & 18.93 & 18.07 & 28.90 & 26.87 & 58.35 & 54.53 & 49.19 & 50.31 & 46.05 & 29.61 \\
\code{bge-base-en-v1.5} & 22.33 & 20.80 & 9.92 & 2.96 & 11.83 & 2.02 & 44.41 & 41.18 & 4.73 & 5.02 & 11.03 & 4.53 & 19.81 & 14.44 & 45.50 & 22.72 & 39.42 & 43.00 & 41.40 & 33.20 \\
\code{bge-large-en-v1.5} & 22.83 & 19.88 & 8.48 & 4.93 & 11.13 & 3.39 & 42.20 & 41.49 & 6.68 & 4.65 & 11.07 & 8.51 & 19.70 & 11.24 & 52.70 & 26.41 & 47.58 & 46.27 & 45.54 & 8.52 \\
\code{text-embedding-3-small} & 23.67 & 22.94 & 14.78 & 12.61 & 19.80 & 17.15 & 40.67 & 33.66 & 10.44 & 9.43 & 13.65 & 11.72 & 24.65 & 22.26 & 57.78 & 58.00 & 46.55 & 46.65 & 47.52 & 45.88 \\
\midrule

\code{e5-mistral-7b-instruct} & 25.48 & 25.42 & 14.81 & 18.83 & 24.48 & 19.68 & 53.54 & 51.35 & 11.62 & 11.82 & 22.26 & 34.95 & 25.82 & 27.36 & 68.13 & 68.10 & 61.91 & 65.49 & 46.80 & 54.97 \\
\code{NV-Embed-v1} & 26.15 & 26.27 & 17.99 & 18.90 & 27.62 & 27.05 & 36.92 & 35.60 & 8.54 & 9.32 & 22.26 & 27.49 & 26.55 & 25.29 & 53.74 & 53.60 & 50.91 & 51.53 & 45.29 & 45.35 \\
\code{GritLM-7B} & 26.50 & 26.19 & 21.34 & 20.75 & 14.25 & 24.23 & 45.98 & 49.93 & 10.23 & 9.99 & 32.68 & 38.82 & 15.97 & 31.05 & 63.87 & 60.14 & 66.08 & 67.15 & 21.53 & 45.39 \\
\code{gte-Qwen2-1.5B-instruct} & 24.90 & 22.42 & 10.35 & 19.92 & 17.15 & 24.88 & 37.20 & 20.44 & 9.30 & 10.18 & 20.82 & 17.42 & 28.14 & 29.66 & 69.37 & 65.72 & 55.67 & 59.61 & 43.16 & 57.27 \\
\midrule

\code{monot5-base-msmarco} & 14.43 & 12.04 & 14.39 & 10.71 & 25.77 & 21.33 & 25.39 & 17.70 & 6.42 & 6.31 & 9.90 & 11.57 & 26.38 & 12.89 & 52.68 & 48.45 & 29.13 & 28.32 & 49.14 & 39.04 \\
\code{bge-reranker-v2-m3} & 15.72 & 5.30 & 7.41 & 4.22 & 19.32 & 15.26 & 24.14 & 20.96 & 6.53 & 10.48 & 24.04 & 22.30 & 36.41 & 29.83 & 46.01 & 27.82 & 45.72 & 36.35 & 56.52 & 54.67 \\
\code{bge-reranker-v2-gemma} & 24.01 & 15.20 & 14.29 & 13.88 & 28.56 & 15.21 & 36.90 & 25.00 & 9.23 & 7.48 & 33.41 & 34.82 & 34.43 & 17.64 & 53.49 & 18.24 & 24.72 & 32.28 & 58.43 & 38.18 \\
\code{jina-reranker-v2-base} & 19.66 & 21.42 & 18.94 & 16.88 & 22.48 & 12.65 & 46.73 & 43.48 & 10.68 & 11.73 & 16.41 & 15.96 & 36.00 & 30.27 & 52.32 & 48.71 & 47.81 & 48.16 & 58.81 & 52.99 \\
\code{mxbai-rerank-large-v1} & 13.38 & 13.67 & 10.88 & 8.82 & 30.59 & 16.28 & 17.10 & 8.12 & 4.89 & 3.98 & 9.06 & 7.33 & 30.40 & 12.41 & 36.33 & 21.70 & 46.67 & 17.77 & 57.83 & 38.73 \\
\code{gpt-3.5-turbo} & 22.76 & 24.69 & 14.55 & 14.13 & 26.58 & 26.19 & 38.97 & 39.19 & 9.52 & 8.79 & 13.38 & 21.49 & 41.50 & 43.51 & 58.45 & 55.88 & 48.40 & 47.95 & 44.89 & 44.28 \\
\bottomrule






\\
\toprule
\textbf{Model} & \multicolumn{2}{c}{\textbf{CPCD}} & \multicolumn{2}{c}{\textbf{ChroniQA}} & \multicolumn{2}{c}{\textbf{NTCIR}} & \multicolumn{2}{c}{\textbf{TableSearch}} & \multicolumn{2}{c}{\textbf{CARE}} & \multicolumn{2}{c}{\textbf{MISeD}} & \multicolumn{2}{c}{\textbf{Spider-SQL}} & \multicolumn{2}{c}{\textbf{LitSearch}} & \multicolumn{2}{c}{\textbf{PM\_19}} & \multicolumn{2}{c}{\textbf{PM-Article\_19}} \\
\midrule
Instruction? & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} \\
\midrule
BM25 & 1.15 & - & 78.77 & - & 25.28 & - & 11.31 & - & 74.10 & - & 60.31 & - & 65.45 & - & 78.41 & - & 49.22 & - & 50.12 & - \\
\midrule

\code{contriever-msmarco} & 2.09 & - & 55.74 & - & 16.66 & - & 13.23 & - & 51.07 & - & 63.61 & - & 54.95 & - & 52.72 & - & 26.99 & - & 35.13 & - \\
\code{gtr-t5-base} & 1.98 & - & 39.91 & - & 12.06 & - & 12.12 & - & 34.23 & - & 55.83 & - & 14.53 & - & 50.31 & - & 27.63 & - & 37.09 & - \\
\code{gtr-t5-large} & 4.77 & - & 40.85 & - & 12.07 & - & 14.05 & - & 33.41 & - & 60.80 & - & 34.84 & - & 53.84 & - & 25.60 & - & 39.07 & - \\
\midrule

\code{all-MiniLM-L6-v2} & 0.26 & 0.19 & 36.13 & 5.89 & 15.06 & 10.19 & 12.01 & 7.27 & 36.66 & 17.11 & 57.14 & 53.14 & 22.97 & 15.81 & 63.23 & 46.63 & 27.59 & 1.97 & 44.99 & 5.74 \\
\code{e5-small-v2} & 4.71 & 2.31 & 56.09 & 47.41 & 12.88 & 8.67 & 9.97 & 8.46 & 54.50 & 44.04 & 54.83 & 51.81 & 50.65 & 33.50 & 49.71 & 29.59 & 25.73 & 5.92 & 40.51 & 14.86 \\
\code{e5-base-v2} & 4.60 & 1.90 & 52.83 & 51.03 & 10.62 & 9.65 & 10.39 & 11.15 & 52.41 & 32.11 & 59.75 & 56.68 & 55.78 & 51.13 & 61.80 & 34.37 & 38.38 & 8.78 & 42.43 & 23.89 \\
\code{e5-large-v2} & 3.98 & 3.70 & 59.53 & 49.61 & 15.21 & 8.08 & 11.92 & 10.45 & 65.37 & 56.72 & 59.30 & 55.90 & 56.07 & 47.04 & 63.43 & 47.24 & 36.32 & 14.19 & 44.67 & 25.07 \\
\code{gte-base-en-v1.5} & 1.03 & 0.14 & 48.87 & 23.69 & 13.18 & 8.32 & 11.83 & 10.81 & 62.60 & 50.82 & 56.18 & 54.99 & 34.70 & 8.54 & 68.51 & 60.15 & 32.12 & 21.18 & 44.25 & 25.77 \\
\code{gte-large-en-v1.5} & 1.02 & 0.30 & 48.95 & 26.65 & 15.62 & 6.98 & 17.89 & 11.64 & 58.40 & 28.73 & 58.23 & 53.33 & 26.53 & 6.06 & 72.30 & 69.52 & 39.78 & 13.03 & 50.06 & 22.12 \\
\code{bge-base-en-v1.5} & 1.03 & 0.17 & 38.68 & 18.79 & 10.55 & 5.88 & 12.22 & 9.02 & 60.20 & 33.52 & 57.24 & 54.32 & 33.67 & 19.31 & 56.80 & 35.44 & 35.51 & 21.27 & 46.59 & 19.21 \\
\code{bge-large-en-v1.5} & 0.62 & 0.24 & 42.52 & 9.98 & 11.75 & 6.87 & 12.45 & 6.97 & 63.76 & 31.22 & 56.85 & 50.12 & 37.21 & 7.86 & 67.34 & 43.48 & 33.57 & 4.44 & 48.70 & 7.21 \\
\code{text-embedding-3-small} & 2.66 & 2.47 & 47.70 & 39.94 & 16.73 & 14.25 & 12.90 & 12.96 & 51.91 & 40.69 & 60.29 & 57.43 & 48.93 & 36.35 & 67.66 & 58.97 & 37.83 & 23.38 & 46.91 & 42.13 \\
\midrule

\code{e5-mistral-7b-instruct} & 2.97 & 4.92 & 53.88 & 48.35 & 19.07 & 16.93 & 14.65 & 14.24 & 72.70 & 68.36 & 62.62 & 60.15 & 65.10 & 62.62 & 69.64 & 78.32 & 38.29 & 45.00 & 53.36 & 54.26 \\
\code{NV-Embed-v1} & 2.20 & 4.06 & 64.72 & 65.47 & 21.79 & 19.76 & 15.34 & 16.33 & 42.97 & 30.79 & 62.66 & 61.03 & 58.96 & 56.91 & 77.02 & 77.44 & 24.39 & 25.47 & 24.03 & 25.74 \\
\code{GritLM-7B} & 6.81 & 8.18 & 34.05 & 61.32 & 3.12 & 16.56 & 12.34 & 13.94 & 58.52 & 50.18 & 59.50 & 61.75 & 52.36 & 59.60 & 71.97 & 74.13 & 44.18 & 55.36 & 48.25 & 51.86 \\
\code{gte-Qwen2-1.5B-instruct} & 3.19 & 5.10 & 55.65 & 50.29 & 16.13 & 19.68 & 14.06 & 16.30 & 65.55 & 58.44 & 61.56 & 59.08 & 44.10 & 41.66 & 74.04 & 76.27 & 25.55 & 19.88 & 54.00 & 50.91 \\
\midrule

\code{monot5-base-msmarco} & 3.78 & 3.16 & 70.81 & 66.58 & 23.24 & 20.40 & 12.43 & 13.53 & 26.73 & 18.84 & 58.36 & 50.45 & 59.57 & 54.95 & 76.77 & 70.66 & 38.28 & 20.74 & 39.89 & 30.58 \\
\code{bge-reranker-v2-m3} & 2.21 & 3.21 & 71.89 & 70.89 & 19.55 & 19.38 & 16.60 & 12.67 & 43.70 & 17.56 & 65.98 & 57.57 & 62.04 & 43.36 & 81.47 & 78.33 & 44.43 & 16.68 & 46.12 & 29.26 \\
\code{bge-reranker-v2-gemma} & 1.81 & 2.54 & 71.51 & 55.10 & 20.05 & 11.85 & 14.24 & 11.34 & 48.77 & 15.88 & 63.73 & 44.78 & 60.54 & 52.58 & 82.03 & 32.97 & 46.58 & 31.14 & 55.32 & 34.11 \\
\code{jina-reranker-v2-base} & 4.51 & 4.23 & 71.42 & 68.23 & 28.98 & 16.01 & 15.04 & 13.79 & 49.15 & 46.09 & 61.78 & 55.33 & 58.21 & 55.21 & 80.24 & 73.30 & 47.82 & 39.86 & 48.63 & 46.68 \\
\code{mxbai-rerank-large-v1} & 2.07 & 4.43 & 65.07 & 34.51 & 20.66 & 12.74 & 14.11 & 11.89 & 48.84 & 16.02 & 61.73 & 47.73 & 60.34 & 3.03 & 83.73 & 11.71 & 37.23 & 26.73 & 48.45 & 38.55 \\
\code{gpt-3.5-turbo} & 5.76 & 5.23 & 62.34 & 61.11 & 16.71 & 17.39 & 13.27 & 12.68 & 49.63 & 44.87 & 61.24 & 62.17 & 37.88 & 41.74 & 70.70 & 71.28 & 42.05 & 39.51 & 47.02 & 47.95 \\
\bottomrule






\\
\toprule
\textbf{Model} & \multicolumn{2}{c}{\textbf{CliniDS\_16}} & \multicolumn{2}{c}{\textbf{CliniTrial\_23}} & \multicolumn{2}{c}{\textbf{Genomics\_07}} & \multicolumn{2}{c}{\textbf{TREC-Legal\_11}} & \multicolumn{2}{c}{\textbf{PytorchAPI}} & \multicolumn{2}{c}{\textbf{Core17}} & \multicolumn{2}{c}{\textbf{News21}} & \multicolumn{2}{c}{\textbf{Robust04}} & \multicolumn{2}{c}{\textbf{NevIR}} & \multicolumn{2}{c}{\textbf{IFEval}} \\
\midrule
Instruction? & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} \\
\midrule
BM25 & 20.79 & - & 44.86 & - & 42.61 & - & 53.87 & - & 67.05 & - & 11.51 & - & 20.79 & - & 18.57 & - & 66.76 & - & 28.28 & - \\
\midrule

\code{contriever-msmarco} & 6.71 & - & 27.10 & - & 23.61 & - & 40.12 & - & 56.50 & - & 18.18 & - & 27.33 & - & 26.64 & - & 62.97 & - & 25.51 & - \\
\code{gtr-t5-base} & 11.68 & - & 23.49 & - & 20.16 & - & 45.90 & - & 46.77 & - & 22.73 & - & 22.49 & - & 26.90 & - & 63.14 & - & 22.59 & - \\
\code{gtr-t5-large} & 12.26 & - & 25.27 & - & 23.66 & - & 47.26 & - & 46.58 & - & 22.80 & - & 26.62 & - & 29.07 & - & 59.95 & - & 23.46 & - \\
\midrule

\code{all-MiniLM-L6-v2} & 11.95 & 9.33 & 22.19 & 5.24 & 20.45 & 10.50 & 49.94 & 15.65 & 39.58 & 36.41 & 20.46 & 17.50 & 26.86 & 25.76 & 25.96 & 23.92 & 57.43 & 41.58 & 26.06 & 37.39 \\
\code{e5-small-v2} & 5.57 & 5.47 & 22.00 & 14.68 & 25.23 & 12.40 & 22.38 & 12.24 & 48.58 & 43.92 & 22.84 & 20.45 & 28.35 & 24.02 & 23.85 & 19.90 & 62.58 & 60.99 & 21.75 & 36.96 \\
\code{e5-base-v2} & 7.69 & 7.17 & 29.39 & 24.80 & 26.21 & 9.90 & 30.08 & 20.34 & 54.26 & 53.61 & 21.62 & 21.03 & 22.92 & 22.17 & 24.32 & 21.09 & 63.96 & 55.68 & 24.47 & 40.33 \\
\code{e5-large-v2} & 10.14 & 10.51 & 27.69 & 19.05 & 30.90 & 22.05 & 22.52 & 10.80 & 61.35 & 57.93 & 22.97 & 29.12 & 25.27 & 26.02 & 29.03 & 23.89 & 66.60 & 62.25 & 22.49 & 39.28 \\
\code{gte-base-en-v1.5} & 21.96 & 22.41 & 26.23 & 9.28 & 32.71 & 12.66 & 53.70 & 11.66 & 56.45 & 53.93 & 21.75 & 21.44 & 25.63 & 22.60 & 27.57 & 25.52 & 58.48 & 41.88 & 25.96 & 42.18 \\
\code{gte-large-en-v1.5} & 26.47 & 28.12 & 32.92 & 13.81 & 30.60 & 13.98 & 47.01 & 23.70 & 46.72 & 39.45 & 27.61 & 26.58 & 25.16 & 26.22 & 30.68 & 29.14 & 58.95 & 45.56 & 25.30 & 41.23 \\
\code{bge-base-en-v1.5} & 18.99 & 16.69 & 23.12 & 16.85 & 29.17 & 13.43 & 29.81 & 29.52 & 54.82 & 50.76 & 19.00 & 20.63 & 21.23 & 20.60 & 23.22 & 19.50 & 63.74 & 48.69 & 24.42 & 36.48 \\
\code{bge-large-en-v1.5} & 17.52 & 18.96 & 23.24 & 11.77 & 31.51 & 3.60 & 49.01 & 24.68 & 59.26 & 58.25 & 24.05 & 18.26 & 21.41 & 22.37 & 27.65 & 19.16 & 64.42 & 36.28 & 22.43 & 37.65 \\
\code{text-embedding-3-small} & 15.75 & 19.23 & 29.07 & 25.04 & 27.40 & 24.64 & 49.19 & 9.37 & 62.07 & 56.56 & 27.57 & 30.04 & 26.22 & 25.60 & 32.19 & 28.15 & 69.06 & 61.44 & 21.50 & 31.91 \\
\midrule

\code{e5-mistral-7b-instruct} & 17.01 & 32.32 & 37.39 & 40.16 & 33.58 & 32.03 & 56.16 & 54.23 & 65.93 & 65.26 & 21.85 & 33.41 & 29.35 & 31.74 & 30.44 & 36.05 & 64.59 & 62.30 & 24.98 & 32.15 \\
\code{NV-Embed-v1} & 13.65 & 18.47 & 31.02 & 32.61 & 30.57 & 32.31 & 43.19 & 45.55 & 64.07 & 66.11 & 26.49 & 32.81 & 33.11 & 30.94 & 33.04 & 35.13 & 69.55 & 69.54 & 22.45 & 27.68 \\
\code{GritLM-7B} & 23.08 & 31.11 & 36.78 & 38.81 & 32.02 & 31.17 & 38.15 & 54.02 & 60.28 & 64.38 & 14.47 & 34.94 & 21.87 & 31.03 & 29.93 & 38.27 & 59.49 & 71.53 & 22.03 & 38.73 \\
\code{gte-Qwen2-1.5B-instruct} & 15.70 & 22.71 & 28.38 & 24.54 & 45.94 & 43.19 & 28.41 & 45.39 & 61.78 & 65.97 & 21.52 & 32.65 & 24.36 & 31.77 & 30.06 & 33.79 & 65.28 & 65.38 & 21.85 & 42.76 \\
\midrule

\code{monot5-base-msmarco} & 9.95 & 11.95 & 18.77 & 15.64 & 28.08 & 31.23 & 54.47 & 46.93 & 26.55 & 20.80 & 28.99 & 18.98 & 26.21 & 14.77 & 32.51 & 24.70 & 76.94 & 75.70 & 24.71 & 31.17 \\
\code{bge-reranker-v2-m3} & 18.11 & 12.56 & 33.50 & 19.29 & 33.57 & 28.16 & 51.13 & 34.77 & 35.74 & 17.76 & 28.17 & 26.80 & 27.31 & 27.06 & 33.91 & 31.80 & 81.92 & 79.06 & 20.86 & 21.23 \\
\code{bge-reranker-v2-gemma} & 21.64 & 17.96 & 33.33 & 21.17 & 33.33 & 18.70 & 55.60 & 40.85 & 75.21 & 64.37 & 28.28 & 29.02 & 31.41 & 27.62 & 39.11 & 30.19 & 80.84 & 65.00 & 19.42 & 53.73 \\
\code{jina-reranker-v2-base} & 20.43 & 19.73 & 37.24 & 31.54 & 54.01 & 53.20 & 64.38 & 52.93 & 64.47 & 64.79 & 26.68 & 31.53 & 29.13 & 30.20 & 32.99 & 34.68 & 79.29 & 75.07 & 11.17 & 20.80 \\
\code{mxbai-rerank-large-v1} & 11.21 & 12.24 & 31.13 & 20.68 & 58.62 & 32.65 & 37.45 & 16.36 & 31.87 & 13.11 & 32.60 & 25.82 & 30.64 & 14.58 & 33.05 & 19.53 & 83.53 & 48.47 & 17.13 & 27.74 \\
\code{gpt-3.5-turbo} & 15.14 & 15.77 & 28.83 & 30.37 & 25.99 & 27.20 & 52.86 & 52.30 & 71.73 & 68.42 & 29.09 & 33.43 & 29.62 & 30.27 & 29.06 & 29.73 & 76.96 & 72.50 & 15.15 & 29.04 \\
\bottomrule
\end{tabular}
\end{table*}


==> table/hard_set_avg.tex <==
\begin{table}[th]
\centering\small
\setlength\tabcolsep{5pt}
\begin{tabular}{l cc cc}

\toprule
\textbf{Model} &  \\
\midrule
Instruction?  & \ding{55} & \ding{51} & \ding{55} & \ding{51} \\
\midrule

BM25 & 40.76 & - & 42.70 & -  \\
% \code{contriever-msmarco} & 33.14 & -  \\
% gtr-t5-base & 29.24 & -  \\
% gtr-t5-large & 31.08 & -  \\
% \code{all-MiniLM-L6-v2} & 29.15 & 21.26  \\
% \code{e5-small-v2} & 31.86 & 27.50  \\
\code{e5-base-v2} & 43.36 & 38.83 & 33.87 & 29.77  \\
\code{e5-large-v2} & 44.69 & 39.42 & 36.25 & 32.37  \\
% gte-base-en-v1.5 & 35.69 & 29.80  \\
% gte-large-en-v1.5 & 36.29 & 28.29  \\
% bge-base-en-v1.5 & 32.70 & 24.59  \\
% bge-large-en-v1.5 & 34.69 & 23.00  \\
\code{text-embedding-3} & 46.47 & 43.90 & 36.33 & 33.04  \\
\code{e5-mistral-7b} & 50.80 & 54.36 & 41.88 & 43.13  \\
\code{NV-Embed-v1} & 50.24 & 51.19 & 37.60 & 37.45  \\
\code{GritLM-7B} & 48.40 & 55.20 & 36.93 & 43.14  \\
\code{gte-Qwen2-1.5B} & 49.09 & 51.76 & 38.47 & 40.07  \\
% monot5-base-msmarco & 32.96 & 28.98  \\
\code{bge-reranker-m3} & 46.56 & 40.42 & 36.38 & 28.84  \\
\code{bge-reranker-gemma} & 52.28 & 38.14 & 40.07 & 29.71  \\
% jina-reranker-v2-base & 40.31 & 38.10  \\
% mxbai-rerank-large-v1 & 35.44 & 18.90  \\
\code{gpt-3.5-turbo} & 47.80 & 48.97 & 38.02 & 38.70  \\
\bottomrule
\end{tabular}
\caption{\textbf{Main Results (nDCG@10)} Rows marked with \ding{51} indicate results with instruction input, while rows marked with \ding{55} indicate results without instruction input. Models labeled with $^\spadesuit$ are instruction fine-tuned. The last group represents the re-ranking models, which all re-rank the top 100 results of \code{text-embedding-3-small}.}
\label{table:main-results}
\end{table}









